Foundational Challenges in Assuring Alignment and Safety of Large Language Models

This work identifies 18 foundational challenges in assuring the alignment and safety of large language models (LLMs). These challenges are organized into three different categories: scientific understanding of LLMs, development and deployment methods, and sociotechnical challenges. Based on the identified challenges, we pose $200+$ concrete research questions.

==> intros/Reader_s_Guide.tex <==
\section*{Reader's Guide}

Due to the length of this document (though note that the main content is only \textasciitilde{}100 pages; the rest are references), it may not be feasible for all readers to go through this document entirely. Hence, we suggest some reading strategies and advice here to help readers better make use of this document.

We recommend all readers begin this document by reading the main introduction (Section~\ref{mainsec:introduction}) to grasp the high-level context of this document. To get a quick overview, readers could browse the introductions to various categories of the challenges (i.e.\ Sections~\ref{mainsec2:insufficient_scientific_understanding_of_llms},\ref{mainsec3:lacking_development_and_deployment_methods} and \ref{mainsec4:sociotechnical_challenges}) and review associated Tables~\ref{table:section_2},~\ref{table:section_3}~and~\ref{table:section_4} that provide a highly abridged overview of the challenges discussed in the three categories.  From there on, readers interested in a deep dive could pick any section of interest. Note that all the challenges (i.e.\ subsections like Section~\ref{sec1:black_box_nature_of_in_context_learning}) are self-contained and thus can be read in an arbitrary order. 

% This document also provides a broad overview of the state of LLM alignment and safety as of the beginning of 2024.
% However, the field moves very quickly, so some parts may be quickly outdated.
% Still, by focusing on fundamental challenges, we hope this work can stand the test of time and serve as a useful guide for years to come.
% For readers seeking a high-level understanding of which challenges need to be addressed to advance LLM alignment and safety, reading the introductory paragraphs of each challenge might be a good way to start engaging with the agenda.

\subsectionnormalsize*{Machine Learning and NLP Researchers}
Technical researchers in machine learning, natural language processing, and other associated fields are the primary intended audience for this agenda. We have tried to assume as minimal background knowledge as possible beyond the general knowledge of what LLMs are, what their architecture is, and how they are trained. Hence, we expect all the technical challenges in Sections~\ref{mainsec2:insufficient_scientific_understanding_of_llms}~and~\ref{mainsec3:lacking_development_and_deployment_methods} to be accessible to any person with the knowledge equivalent to a first-year graduate student in machine learning or natural language processing. A large proportion of the challenges discussed in Section~\ref{mainsec4:sociotechnical_challenges} are also technical in nature and should be equally accessible.

The main intended purpose of this document is to help junior researchers, or researchers new to this area, to identify promising and actionable research directions (although of course, even seasoned experts might take inspiration from it).
Such readers are encouraged to pick and choose sections that best align with their interests.
The 200\plusop\, listed research questions are each meant to be roughly the size of a problem that could form the basis of a research dissertation.
For each challenge and subchallenge, we provide motivation, background, and related work, before discussing directions for future research.
These should provide a good starting point for researchers who are new to these particular challenges, but we do not attempt a comprehensive survey of any area.

We also note that while this work is motivated by the safety and alignment of LLMs, nonetheless, many of the challenges we identify are highly interesting from the technical and scientific points of view. Thus, even those readers who are not primarily motivated by safety, but are in search of interesting problems centered on LLMs, may find this document useful.

\subsectionnormalsize*{Sociotechnical Researchers and Other Stakeholders}
We focus on sociotechnical challenges in Section~\ref{mainsec4:sociotechnical_challenges}, but emphasize that all LLMs are sociotechnical systems, and their safety cannot be ensured without a deep and thoughtful consideration through this lens. The introduction of this section provides a mapping between the different challenges we discuss and the different areas of other fields that could contribute to progress on those challenges. This section only presumes high-level familiarity with the LLMs for the most part, and is aimed to be accessible to a wider audience than the rest of the agenda. 
% As primarily technical researchers ourselves, we do not attempt to be comprehensive in this section of the very wide array of sociotechnical challenges LLMs may pose.  Rather, the intention in this section is to help build the necessary bridges to enable meaningful participation of a more diverse set of stakeholders than are typically included in research on LLM alignment and safety.

